Multigrid Neural Architectures

We propose a multigrid extension of convolutional neural networks (CNNs). Rather than manipulating representations living on a single spatial grid, our network layers operate across scale space, on a pyramid of grids. They consume multigrid inputs and produce multigrid outputs; convolutional filters themselves have both within-scale and cross-scale extent. This aspect is distinct from simple multiscale designs, which only process the input at different scales. Viewed in terms of information flow, a multigrid network passes messages across a spatial pyramid. As a consequence, receptive field size grows exponentially with depth, facilitating rapid integration of context. Most critically, multigrid structure enables networks to learn internal attention and dynamic routing mechanisms, and use them to accomplish tasks on which modern CNNs fail. Experiments demonstrate wide-ranging performance advantages of multigrid. On CIFAR and ImageNet classification tasks, flipping from a single grid to multigrid within the standard CNN paradigm improves accuracy, while being compute and parameter efficient. Multigrid is independent of other architectural choices; we show synergy in combination with residual connections. Multigrid yields dramatic improvement on a synthetic semantic segmentation dataset. Most strikingly, relatively shallow multigrid networks can learn to directly perform spatial transformation tasks, where, in contrast, current CNNs fail. Together, our results suggest that continuous evolution of features on a multigrid pyramid is a more powerful alternative to existing CNN designs on a flat grid.

==> Makefile <==
# programs
PDFLATEX = pdflatex
CP       = cp
RM       = rm
GREP     = grep
DIFF     = diff -q
TOUCH    = touch

# input and output files
TEXFILE = nmg_arxiv.tex
PDFFILE = nmg_arxiv.pdf
TEXINCLUDES = $(wildcard include/*)

# intermediate files
TEXLOG     = $(basename $(TEXFILE)).log
AUXFILE    = $(basename $(TEXFILE)).aux
OLDAUXFILE = $(AUXFILE).old

# arxiv submission files
ARXIV_FILES := $(if $(wildcard files.txt),$(shell cat files.txt),)
ARXIV_OUT   := arxiv.tar.gz

# If this message appears in TEXLOG, we must re-run LaTeX.
RERUNLATEX = "Rerun to get cross-references right"

# The primary target (created by the command "make") is the PDF file.
.PHONY: pdf
pdf: $(PDFFILE)

# This rule uses PDFLaTeX to create a PDF file from a LaTeX file.
# Then PDFLaTeX is re-run to resolve references, as necessary.
$(PDFFILE): $(TEXFILE) $(TEXINCLUDES)
	$(TOUCH) $(AUXFILE)
	$(CP) $(AUXFILE) $(OLDAUXFILE)
	$(PDFLATEX) $<
	while $(GREP) -q $(RERUNLATEX) $(TEXLOG); do $(PDFLATEX) $<; done

# arxiv submission
.PHONY: submit
submit: $(ARXIV_OUT)
$(ARXIV_OUT): files.txt $(ARXIV_FILES)
	@COPYFILE_DISABLE=1 tar cvzfh $(ARXIV_OUT) $(ARXIV_FILES)

# This rule cleans out the files made by the make process.
clean:
	$(RM) -f $(AUXFILE)\
                 $(OLDAUXFILE)\
                 $(TEXLOG)\
                 $(PDFFILE)\
                 $(ARXIV_OUT)


==> include/nmg/fig_supp_seg_content.tex <==
\setlength\fboxsep{0pt}
\begin{minipage}[t]{0.4975\linewidth}
   \vspace{0pt}
   % example 00156
   \begin{center}
   \begin{minipage}[t]{0.09\linewidth}
      \vspace{0pt}
      \begin{center}
         \tiny{\textbf{\textsf{Input}}}\\
         \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_input.png}}
      \end{center}
   \end{minipage}
   \hfill
   \begin{minipage}[t]{0.90\linewidth}
      \vspace{0pt}
      \begin{center}
         % digits output
         \begin{minipage}[t]{0.94\linewidth}
            \vspace{0pt}
            \begin{center}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{Digit: 0}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_label_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_unet_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmg2_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmg2_0.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}1\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_label_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_unet_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmg2_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmg2_1.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}2\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_label_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_unet_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmg2_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmg2_2.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}3\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_label_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_unet_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmg2_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmg2_3.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}4\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_label_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_unet_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmg2_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmg2_4.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}5\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_label_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_unet_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmg2_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmg2_5.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}6\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_label_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_unet_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmg2_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmg2_6.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}7\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_label_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_unet_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmg2_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmg2_7.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}8\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_label_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_unet_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmg2_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmg2_8.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}9\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_label_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_unet_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_pnmg2_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00156_prnmg2_9.png}}
               \end{center}
            \end{minipage}
            \end{center}
         \end{minipage}
         % method labels
         \begin{minipage}[t]{0.04\linewidth}
            \vspace{0pt}
            \begin{rotate}{270}
               \tiny{\textbf{\textsf{
                  \hspace*{8pt}
                  True
                  \hspace*{4pt}
                  U-NET
                  \hspace*{7pt}
                  SG
                  \hspace*{8pt}
                  R-SG
                  \hspace*{6pt}
                  PMG
                  \hspace*{4pt}
                  R-PMG
               }}}
            \end{rotate}
         \end{minipage}
      \end{center}
   \end{minipage}
   \end{center}
\end{minipage}
\hfill
\begin{minipage}[t]{0.4975\linewidth}
   \vspace{0pt}
   % example 00170
   \begin{center}
   \begin{minipage}[t]{0.09\linewidth}
      \vspace{0pt}
      \begin{center}
         \tiny{\textbf{\textsf{Input}}}\\
         \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_input.png}}
      \end{center}
   \end{minipage}
   \hfill
   \begin{minipage}[t]{0.90\linewidth}
      \vspace{0pt}
      \begin{center}
         % digits output
         \begin{minipage}[t]{0.94\linewidth}
            \vspace{0pt}
            \begin{center}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{Digit: 0}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_label_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_unet_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmg2_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmg2_0.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}1\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_label_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_unet_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmg2_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmg2_1.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}2\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_label_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_unet_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmg2_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmg2_2.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}3\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_label_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_unet_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmg2_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmg2_3.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}4\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_label_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_unet_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmg2_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmg2_4.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}5\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_label_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_unet_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmg2_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmg2_5.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}6\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_label_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_unet_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmg2_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmg2_6.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}7\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_label_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_unet_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmg2_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmg2_7.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}8\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_label_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_unet_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmg2_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmg2_8.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}9\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_label_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_unet_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_pnmg2_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00170_prnmg2_9.png}}
               \end{center}
            \end{minipage}
            \end{center}
         \end{minipage}
         % method labels
         \begin{minipage}[t]{0.04\linewidth}
            \vspace{0pt}
            \begin{rotate}{270}
               \tiny{\textbf{\textsf{
                  \hspace*{8pt}
                  True
                  \hspace*{4pt}
                  U-NET
                  \hspace*{7pt}
                  SG
                  \hspace*{8pt}
                  R-SG
                  \hspace*{6pt}
                  PMG
                  \hspace*{4pt}
                  R-PMG
               }}}
            \end{rotate}
         \end{minipage}
      \end{center}
   \end{minipage}
   \end{center}
\end{minipage}\\
\vspace{0.05\linewidth}
\begin{minipage}[t]{0.4975\linewidth}
   \vspace{0pt}
   % example 00171
   \begin{center}
   \begin{minipage}[t]{0.09\linewidth}
      \vspace{0pt}
      \begin{center}
         \tiny{\textbf{\textsf{Input}}}\\
         \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_input.png}}
      \end{center}
   \end{minipage}
   \hfill
   \begin{minipage}[t]{0.90\linewidth}
      \vspace{0pt}
      \begin{center}
         % digits output
         \begin{minipage}[t]{0.94\linewidth}
            \vspace{0pt}
            \begin{center}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{Digit: 0}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_label_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_unet_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmg2_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmg2_0.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}1\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_label_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_unet_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmg2_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmg2_1.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}2\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_label_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_unet_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmg2_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmg2_2.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}3\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_label_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_unet_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmg2_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmg2_3.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}4\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_label_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_unet_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmg2_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmg2_4.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}5\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_label_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_unet_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmg2_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmg2_5.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}6\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_label_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_unet_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmg2_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmg2_6.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}7\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_label_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_unet_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmg2_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmg2_7.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}8\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_label_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_unet_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmg2_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmg2_8.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}9\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_label_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_unet_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_pnmg2_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00171_prnmg2_9.png}}
               \end{center}
            \end{minipage}
            \end{center}
         \end{minipage}
         % method labels
         \begin{minipage}[t]{0.04\linewidth}
            \vspace{0pt}
            \begin{rotate}{270}
               \tiny{\textbf{\textsf{
                  \hspace*{8pt}
                  True
                  \hspace*{4pt}
                  U-NET
                  \hspace*{7pt}
                  SG
                  \hspace*{8pt}
                  R-SG
                  \hspace*{6pt}
                  PMG
                  \hspace*{4pt}
                  R-PMG
               }}}
            \end{rotate}
         \end{minipage}
      \end{center}
   \end{minipage}
   \end{center}
\end{minipage}
\hfill
\begin{minipage}[t]{0.4975\linewidth}
   \vspace{0pt}
   % example 00200
   \begin{center}
   \begin{minipage}[t]{0.09\linewidth}
      \vspace{0pt}
      \begin{center}
         \tiny{\textbf{\textsf{Input}}}\\
         \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_input.png}}
      \end{center}
   \end{minipage}
   \hfill
   \begin{minipage}[t]{0.90\linewidth}
      \vspace{0pt}
      \begin{center}
         % digits output
         \begin{minipage}[t]{0.94\linewidth}
            \vspace{0pt}
            \begin{center}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{Digit: 0}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_label_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_unet_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmg2_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmg2_0.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}1\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_label_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_unet_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmg2_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmg2_1.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}2\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_label_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_unet_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmg2_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmg2_2.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}3\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_label_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_unet_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmg2_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmg2_3.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}4\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_label_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_unet_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmg2_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmg2_4.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}5\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_label_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_unet_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmg2_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmg2_5.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}6\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_label_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_unet_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmg2_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmg2_6.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}7\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_label_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_unet_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmg2_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmg2_7.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}8\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_label_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_unet_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmg2_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmg2_8.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}9\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_label_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_unet_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_pnmg2_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00200_prnmg2_9.png}}
               \end{center}
            \end{minipage}
            \end{center}
         \end{minipage}
         % method labels
         \begin{minipage}[t]{0.04\linewidth}
            \vspace{0pt}
            \begin{rotate}{270}
               \tiny{\textbf{\textsf{
                  \hspace*{8pt}
                  True
                  \hspace*{4pt}
                  U-NET
                  \hspace*{7pt}
                  SG
                  \hspace*{8pt}
                  R-SG
                  \hspace*{6pt}
                  PMG
                  \hspace*{4pt}
                  R-PMG
               }}}
            \end{rotate}
         \end{minipage}
      \end{center}
   \end{minipage}
   \end{center}
\end{minipage}\\
\vspace{0.05\linewidth}
\begin{minipage}[t]{0.4975\linewidth}
   \vspace{0pt}
   % example 00229
   \begin{center}
   \begin{minipage}[t]{0.09\linewidth}
      \vspace{0pt}
      \begin{center}
         \tiny{\textbf{\textsf{Input}}}\\
         \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_input.png}}
      \end{center}
   \end{minipage}
   \hfill
   \begin{minipage}[t]{0.90\linewidth}
      \vspace{0pt}
      \begin{center}
         % digits output
         \begin{minipage}[t]{0.94\linewidth}
            \vspace{0pt}
            \begin{center}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{Digit: 0}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_label_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_unet_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmg2_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmg2_0.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}1\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_label_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_unet_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmg2_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmg2_1.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}2\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_label_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_unet_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmg2_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmg2_2.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}3\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_label_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_unet_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmg2_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmg2_3.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}4\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_label_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_unet_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmg2_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmg2_4.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}5\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_label_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_unet_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmg2_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmg2_5.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}6\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_label_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_unet_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmg2_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmg2_6.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}7\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_label_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_unet_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmg2_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmg2_7.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}8\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_label_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_unet_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmg2_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmg2_8.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}9\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_label_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_unet_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_pnmg2_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00229_prnmg2_9.png}}
               \end{center}
            \end{minipage}
            \end{center}
         \end{minipage}
         % method labels
         \begin{minipage}[t]{0.04\linewidth}
            \vspace{0pt}
            \begin{rotate}{270}
               \tiny{\textbf{\textsf{
                  \hspace*{8pt}
                  True
                  \hspace*{4pt}
                  U-NET
                  \hspace*{7pt}
                  SG
                  \hspace*{8pt}
                  R-SG
                  \hspace*{6pt}
                  PMG
                  \hspace*{4pt}
                  R-PMG
               }}}
            \end{rotate}
         \end{minipage}
      \end{center}
   \end{minipage}
   \end{center}
\end{minipage}
\hfill
\begin{minipage}[t]{0.4975\linewidth}
   \vspace{0pt}
   % example 00240
   \begin{center}
   \begin{minipage}[t]{0.09\linewidth}
      \vspace{0pt}
      \begin{center}
         \tiny{\textbf{\textsf{Input}}}\\
         \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_input.png}}
      \end{center}
   \end{minipage}
   \hfill
   \begin{minipage}[t]{0.90\linewidth}
      \vspace{0pt}
      \begin{center}
         % digits output
         \begin{minipage}[t]{0.94\linewidth}
            \vspace{0pt}
            \begin{center}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{Digit: 0}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_label_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_unet_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmg2_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmg2_0.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}1\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_label_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_unet_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmg2_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmg2_1.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}2\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_label_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_unet_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmg2_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmg2_2.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}3\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_label_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_unet_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmg2_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmg2_3.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}4\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_label_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_unet_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmg2_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmg2_4.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}5\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_label_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_unet_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmg2_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmg2_5.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}6\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_label_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_unet_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmg2_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmg2_6.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}7\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_label_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_unet_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmg2_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmg2_7.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}8\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_label_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_unet_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmg2_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmg2_8.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}9\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_label_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_unet_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_pnmg2_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00240_prnmg2_9.png}}
               \end{center}
            \end{minipage}
            \end{center}
         \end{minipage}
         % method labels
         \begin{minipage}[t]{0.04\linewidth}
            \vspace{0pt}
            \begin{rotate}{270}
               \tiny{\textbf{\textsf{
                  \hspace*{8pt}
                  True
                  \hspace*{4pt}
                  U-NET
                  \hspace*{7pt}
                  SG
                  \hspace*{8pt}
                  R-SG
                  \hspace*{6pt}
                  PMG
                  \hspace*{4pt}
                  R-PMG
               }}}
            \end{rotate}
         \end{minipage}
      \end{center}
   \end{minipage}
   \end{center}
\end{minipage}\\
\vspace{0.05\linewidth}
\begin{minipage}[t]{0.4975\linewidth}
   \vspace{0pt}
   % example 00269
   \begin{center}
   \begin{minipage}[t]{0.09\linewidth}
      \vspace{0pt}
      \begin{center}
         \tiny{\textbf{\textsf{Input}}}\\
         \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_input.png}}
      \end{center}
   \end{minipage}
   \hfill
   \begin{minipage}[t]{0.90\linewidth}
      \vspace{0pt}
      \begin{center}
         % digits output
         \begin{minipage}[t]{0.94\linewidth}
            \vspace{0pt}
            \begin{center}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{Digit: 0}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_label_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_unet_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmg2_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmg2_0.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}1\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_label_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_unet_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmg2_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmg2_1.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}2\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_label_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_unet_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmg2_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmg2_2.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}3\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_label_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_unet_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmg2_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmg2_3.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}4\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_label_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_unet_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmg2_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmg2_4.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}5\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_label_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_unet_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmg2_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmg2_5.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}6\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_label_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_unet_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmg2_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmg2_6.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}7\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_label_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_unet_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmg2_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmg2_7.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}8\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_label_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_unet_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmg2_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmg2_8.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}9\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_label_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_unet_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_pnmg2_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00269_prnmg2_9.png}}
               \end{center}
            \end{minipage}
            \end{center}
         \end{minipage}
         % method labels
         \begin{minipage}[t]{0.04\linewidth}
            \vspace{0pt}
            \begin{rotate}{270}
               \tiny{\textbf{\textsf{
                  \hspace*{8pt}
                  True
                  \hspace*{4pt}
                  U-NET
                  \hspace*{7pt}
                  SG
                  \hspace*{8pt}
                  R-SG
                  \hspace*{6pt}
                  PMG
                  \hspace*{4pt}
                  R-PMG
               }}}
            \end{rotate}
         \end{minipage}
      \end{center}
   \end{minipage}
   \end{center}
\end{minipage}
\hfill
\begin{minipage}[t]{0.4975\linewidth}
   \vspace{0pt}
   % example 00304
   \begin{center}
   \begin{minipage}[t]{0.09\linewidth}
      \vspace{0pt}
      \begin{center}
         \tiny{\textbf{\textsf{Input}}}\\
         \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_input.png}}
      \end{center}
   \end{minipage}
   \hfill
   \begin{minipage}[t]{0.90\linewidth}
      \vspace{0pt}
      \begin{center}
         % digits output
         \begin{minipage}[t]{0.94\linewidth}
            \vspace{0pt}
            \begin{center}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{Digit: 0}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_label_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_unet_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmgsg_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmg2_0.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmg2_0.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}1\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_label_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_unet_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmgsg_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmg2_1.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmg2_1.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}2\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_label_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_unet_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmgsg_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmg2_2.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmg2_2.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}3\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_label_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_unet_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmgsg_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmg2_3.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmg2_3.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}4\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_label_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_unet_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmgsg_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmg2_4.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmg2_4.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}5\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_label_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_unet_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmgsg_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmg2_5.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmg2_5.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}6\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_label_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_unet_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmgsg_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmg2_6.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmg2_6.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}7\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_label_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_unet_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmgsg_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmg2_7.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmg2_7.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}8\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_label_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_unet_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmgsg_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmg2_8.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmg2_8.png}}
               \end{center}
            \end{minipage}
            \begin{minipage}[t]{0.09\linewidth}
               \vspace{0pt}
               \begin{center}
               \tiny{\textbf{\textsf{\phantom{g}9\phantom{g}}}}\\
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_label_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_unet_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmgsg_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_pnmg2_9.png}}
               \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-seg/00304_prnmg2_9.png}}
               \end{center}
            \end{minipage}
            \end{center}
         \end{minipage}
         % method labels
         \begin{minipage}[t]{0.04\linewidth}
            \vspace{0pt}
            \begin{rotate}{270}
               \tiny{\textbf{\textsf{
                  \hspace*{8pt}
                  True
                  \hspace*{4pt}
                  U-NET
                  \hspace*{7pt}
                  SG
                  \hspace*{8pt}
                  R-SG
                  \hspace*{6pt}
                  PMG
                  \hspace*{4pt}
                  R-PMG
               }}}
            \end{rotate}
         \end{minipage}
      \end{center}
   \end{minipage}
   \end{center}
\end{minipage}


==> include/nmg/fig_supp_spt_content.tex <==
\setlength\fboxsep{0pt}
% spatial transform examples
\begin{minipage}[t]{1.00\linewidth}
   \vspace{0pt}
   \begin{center}
   \begin{minipage}[t]{0.13143\linewidth}
      \vspace{0pt}
      \begin{center}
      \tiny{\textbf{\textsf{Input}}}\\
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00100_input_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00101_input_3.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00102_input_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00103_input_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00104_input_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00105_input_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00106_input_0.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00107_input_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00108_input_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00109_input_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00110_input_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00111_input_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00112_input_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00113_input_2.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00114_input_1.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00115_input_6.png}}
      \end{center}
   \end{minipage}
   \begin{minipage}[t]{0.13143\linewidth}
      \vspace{0pt}
      \begin{center}
      \tiny{\textbf{\textsf{\phantom{p}True\phantom{p}}}}\\
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00100_label_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00101_label_3.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00102_label_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00103_label_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00104_label_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00105_label_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00106_label_0.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00107_label_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00108_label_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00109_label_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00110_label_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00111_label_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00112_label_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00113_label_2.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00114_label_1.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00115_label_6.png}}
      \end{center}
   \end{minipage}
   \begin{minipage}[t]{0.13143\linewidth}
      \vspace{0pt}
      \begin{center}
      \tiny{\textbf{\textsf{\phantom{p}U-NET\phantom{p}}}}\\
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00100_unet_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00101_unet_3.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00102_unet_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00103_unet_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00104_unet_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00105_unet_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00106_unet_0.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00107_unet_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00108_unet_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00109_unet_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00110_unet_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00111_unet_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00112_unet_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00113_unet_2.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00114_unet_1.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00115_unet_6.png}}
      \end{center}
   \end{minipage}
   \begin{minipage}[t]{0.13143\linewidth}
      \vspace{0pt}
      \begin{center}
      \tiny{\textbf{\textsf{\phantom{p}SG}\phantom{p}}}\\
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00100_pnmgsg_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00101_pnmgsg_3.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00102_pnmgsg_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00103_pnmgsg_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00104_pnmgsg_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00105_pnmgsg_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00106_pnmgsg_0.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00107_pnmgsg_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00108_pnmgsg_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00109_pnmgsg_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00110_pnmgsg_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00111_pnmgsg_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00112_pnmgsg_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00113_pnmgsg_2.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00114_pnmgsg_1.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00115_pnmgsg_6.png}}
      \end{center}
   \end{minipage}
   \begin{minipage}[t]{0.13143\linewidth}
      \vspace{0pt}
      \begin{center}
      \tiny{\textbf{\textsf{\phantom{p}R-SG\phantom{p}}}}\\
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00100_prnmgsg_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00101_prnmgsg_3.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00102_prnmgsg_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00103_prnmgsg_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00104_prnmgsg_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00105_prnmgsg_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00106_prnmgsg_0.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00107_prnmgsg_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00108_prnmgsg_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00109_prnmgsg_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00110_prnmgsg_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00111_prnmgsg_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00112_prnmgsg_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00113_prnmgsg_2.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00114_prnmgsg_1.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00115_prnmgsg_6.png}}
      \end{center}
   \end{minipage}
   \begin{minipage}[t]{0.13143\linewidth}
      \vspace{0pt}
      \begin{center}
      \tiny{\textbf{\textsf{\phantom{p}PMG\phantom{p}}}}\\
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00100_pnmg2_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00101_pnmg2_3.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00102_pnmg2_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00103_pnmg2_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00104_pnmg2_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00105_pnmg2_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00106_pnmg2_0.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00107_pnmg2_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00108_pnmg2_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00109_pnmg2_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00110_pnmg2_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00111_pnmg2_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00112_pnmg2_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00113_pnmg2_2.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00114_pnmg2_1.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00115_pnmg2_6.png}}
      \end{center}
   \end{minipage}
   \begin{minipage}[t]{0.13143\linewidth}
      \vspace{0pt}
      \begin{center}
      \tiny{\textbf{\textsf{\phantom{p}R-PMG\phantom{p}}}}\\
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00100_prnmg2_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00101_prnmg2_3.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00102_prnmg2_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00103_prnmg2_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00104_prnmg2_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00105_prnmg2_2.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00106_prnmg2_0.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00107_prnmg2_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00108_prnmg2_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00109_prnmg2_9.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00110_prnmg2_1.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00111_prnmg2_5.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00112_prnmg2_6.png}}
      \fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00113_prnmg2_2.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00114_prnmg2_1.png}}
      %\fbox{\includegraphics[width=1.0\linewidth]{figures/mnist-spt/00115_prnmg2_6.png}}
      \end{center}
   \end{minipage}\\
   \vspace{0.012\linewidth}
   \end{center}
\end{minipage}

